Analyzing the Language of Food on Social Media

We investigate the predictive power behind the language of food on social media. We collect a corpus of over three million food-related posts from Twitter and demonstrate that many latent population characteristics can be directly predicted from this data: overweight rate, diabetes rate, political leaning, and home geographical location of authors. For all tasks, our language-based models significantly outperform the majority-class baselines. Performance is further improved with more complex natural language processing, such as topic modeling. We analyze which textual features have most predictive power for these datasets, providing insight into the connections between the language of food, geographic locale, and community characteristics. Lastly, we design and implement an online system for real-time query and visualization of the dataset. Visualization tools, such as geo-referenced heatmaps, semantics-preserving wordclouds and temporal histograms, allow us to discover more complex, global patterns mirrored in the language of food.

==> state_weights.tex <==
\begin{table}
        \begin{subtable}{0.25\textwidth}
            \begin{tabular}{l}
                30\\
                \#wgfak\\
                \emph{Wine} (wine, 2014, today)\\
                \#whole\\
                \emph{Paleo Diet} (paleo, chicken, healthy)\\
                \#foodtruck\\
                otis\\
                lake\\
                \#dashadoeswhole\\
                sonho\\
            \end{tabular}
            \caption{        AK }
        \end{subtable}

        \begin{subtable}{0.25\textwidth}
            \begin{tabular}{l}
                my\\
                music\\
                i\\
                \#hustle\\
                food\\
                \#meal\\
                cosmo\\
                \#yummy\\
                \emph{Meat} (steak, beef, meat)\\
                \#food\\
            \end{tabular}
            \caption{        AL }
        \end{subtable}
        \begin{subtable}{0.25\textwidth}
            \begin{tabular}{l}
        \#eatclean\\
        i\\
        \#recipe\\
        love\\
        \#healthyliving\\
        good\\
        \#yum\\
        1\\
        photo\\
        looks\\
    \end{tabular}
    \caption{        AR }
\end{subtable}

\begin{subtable}{0.25\textwidth}
    \begin{tabular}{l}
        dinner\\
        photo\\
        \emph{Recipe} (recipe, easy, meal)\\
        \#easy\\
        \emph{Mexican} (mexican, tacos, burrito)\\
        \#yummy\\
        easy\\
        TOPIC\_110\\
        \#foodie\\
        \#eatclean\\
    \end{tabular}
    \caption{        AZ }
\end{subtable}

\begin{subtable}{0.25\textwidth}
    \begin{tabular}{l}
        \emph{Mexican} (mexican, tacos, burrito)\\
        \#vegan\\
        w\\
        \#vegetarian\\
        my\\
        \#bomb\\
        photo\\
        \emph{Wine} (wine, 2014, today)\\
        TOPIC\_174\\
        \#food\\
    \end{tabular}
    \caption{        CA }
\end{subtable}

\begin{subtable}{0.25\textwidth}
    \begin{tabular}{l}
        w\\
        \#glutenfree\\
        TOPIC\_59\\
        \emph{Turkish} (turkish, kebab, istanbul)9\\
        \emph{You, We} (you, we, your, us)\\
        garlic\\
        oil\\
        \#jellyucafe\\
        special\\
        salad\\
    \end{tabular}
    \caption{        CO }
\end{subtable}

\begin{subtable}{0.25\textwidth}
    \begin{tabular}{l}
        21dayfix\\
        rolls\\
        pink\\
        sumo\\
        TOPIC\_155\\
        \#dinner\\
        \#westhartford\\
        signature\\
        \#specials\\
        \#frantasticallyfit\\
    \end{tabular}
    \caption{        CT }
\end{subtable}

\begin{subtable}{0.25\textwidth}
    \begin{tabular}{l}
        \#brunch\\
        \emph{Restaurant Advertising} (open, today, come, join)\\
        brunch\\
        today\\
        TOPIC\_133\\
        we\\
        come\\
        open\\
        TOPIC\_112\\
        via\\
    \end{tabular}
    \caption{        DC }
\end{subtable}

\begin{subtable}{0.25\textwidth}
    \begin{tabular}{l}
        just\\
        fridays\\
        starting\\
        \#alohamonkeywellness\\
        \#specials\\
        dishes\\
        good\\
        you\\
        \emph{Restaurant Advertising} (open, today, come, join)\\
        day\\
    \end{tabular}
    \caption{        DE }
\end{subtable}

\begin{subtable}{0.25\textwidth}
    \begin{tabular}{l}
        \emph{Vacation} (beach, hotel, vacation)\\
        \#designdistrict\\
        \#family\\
        \#lunch\\
        gigi\\
        TOPIC\_76\\
        \#southbeach\\
        \emph{Roasted Meats} (pork, chicken, special)\\
        \#easter\\
        \emph{Paleo Diet} (paleo, chicken, healthy)7\\
    \end{tabular}
    \caption{        FL }
\end{subtable}

\begin{subtable}{0.25\textwidth}
    \begin{tabular}{l}
        chicken\\
        \#foodie\\
        my\\
        nom\\
        \emph{I, You} (i, my, you, your)\\
        \emph{American Diet} (chicken, beans, potatoes)\\
        \emph{First-Person Casual} (my, i, lol)\\
        grits\\
        \emph{Delicious} (foodporn, yummy, yum)\\
        \#goodeats\\
    \end{tabular}
    \caption{        GA }
\end{subtable}

\begin{subtable}{0.25\textwidth}
    \begin{tabular}{l}
        \emph{Turkish} (turkish, kebab, istanbul)\\
        TOPIC\_120\\
        \#ono\\
        come\\
        \#oishii\\
        down\\
        TOPIC\_175\\
        \#dinner\\
        \#lunch\\
        \#itadakimas\\
    \end{tabular}
    \caption{        HI }
\end{subtable}

\begin{subtable}{0.25\textwidth}
    \begin{tabular}{l}
        \#lunch\\
        \#supper\\
        night\\
        TOPIC\_155\\
        \#foodpic\\
        tonight\\
        my\\
        eating\\
        your\\
        \#pizza\\
    \end{tabular}
    \caption{        IA }
\end{subtable}

\begin{subtable}{0.25\textwidth}
    \begin{tabular}{l}
        TOPIC\_130\\
        \emph{Directions} (west, local, east)9\\
        TOPIC\_146\\
        \#instafood\\
        \#snack\\
        \emph{Paleo Diet} (paleo, chicken, healthy)9\\
        \#shakeology\\
        \#fitmama\\
        \#fitness\\
        \#motivation\\
    \end{tabular}
    \caption{        ID }
\end{subtable}

\begin{subtable}{0.25\textwidth}
    \begin{tabular}{l}
        \emph{Giveaway} (win, competition, enter)\\
        jerk\\
        \#bbq\\
        \emph{You, We} (you, we, your, us)\\
        \#breakfast\\
        \#paleoporn\\
        \#primal\\
        \#foodie\\
        \#jamaican\\
        \#jerkchicken\\
    \end{tabular}
    \caption{        IL }
\end{subtable}

\begin{subtable}{0.25\textwidth}
    \begin{tabular}{l}
        \#recipes\\
        \#delicious\\
        \#meals\\
        \#dinnerideas\\
        TOPIC\_19\\
        \#food\\
        \#foodies\\
        \#mealideas\\
        \#baking\\
        \#cooking\\
    \end{tabular}
    \caption{        IN }
\end{subtable}

\begin{subtable}{0.25\textwidth}
    \begin{tabular}{l}
        \#dessert\\
        i\\
        4\\
        out\\
        morning\\
        so\\
        \emph{Promotional} (free, off, today)\\
        tonight\\
        easy\\
        \emph{I, You} (i, my, you, your)\\
    \end{tabular}
    \caption{        KS }
\end{subtable}

\begin{subtable}{0.25\textwidth}
    \begin{tabular}{l}
        \#taco\\
        \#bell\\
        \#supper\\
        \emph{Mexican} (mexican, tacos, burrito)\\
        \emph{After Work} (time, home, after, work)\\
        \#usa\\
        my\\
        \#breakfast\\
        \#mcdonald\\
        love\\
    \end{tabular}
    \caption{        KY }
\end{subtable}

\begin{subtable}{0.25\textwidth}
    \begin{tabular}{l}
        \#foodporn\\
        \#nola\\
        \#food\\
        \#instafood\\
        \emph{American Diet} (chicken, beans, potatoes)\\
        special\\
        \#lunch\\
        \#yummy\\
        \#yum\\
        \#foodie\\
    \end{tabular}
    \caption{        LA }
\end{subtable}

\begin{subtable}{0.25\textwidth}
    \begin{tabular}{l}
        \#diet\\
        \#fitness\\
        \#fitnessnutrition\\
        \#meal\\
        \emph{Roasted Meats} (pork, chicken, special)\\
        our\\
        \#food\\
        \#nbpt\\
        we\\
        TOPIC\_123\\
    \end{tabular}
    \caption{        MA }
\end{subtable}

\begin{subtable}{0.25\textwidth}
    \begin{tabular}{l}
        \#taco\\
        \#bento\\
        \#bell\\
        \#justbento\\
        \#eco\\
        \emph{Restaurant Advertising} (open, today, come, join)\\
        TOPIC\_109\\
        \#foodgasm\\
        \#food\\
        bento\\
    \end{tabular}
    \caption{        MD }
\end{subtable}
\begin{subtable}{0.25\textwidth}
    \begin{tabular}{l}
        \#dinner\\
        \emph{After Work} (time, home, after, work)\\
        \#foodporn\\
        \#love\\
        \#thegothicrestaurant\\
        n\\
        \emph{Japanese} (ramen, japanese, noodles)7\\
        TOPIC\_87\\
        \#party\\
        TOPIC\_154\\
    \end{tabular}
    \caption{        ME }
\end{subtable}

\begin{subtable}{0.25\textwidth}
    \begin{tabular}{l}
        \#breakfast\\
        TOPIC\_138\\
        \emph{Meat} (steak, beef, meat)6\\
        \#superbowl\\
        5\\
        \#do\\
        度\\
        tasty\\
        4sup\\
        \#recipes\\
    \end{tabular}
    \caption{        MI }
\end{subtable}

\begin{subtable}{0.25\textwidth}
    \begin{tabular}{l}
        make\\
        our\\
        \#cooking\\
        \#mpls\\
        chicken\\
        \#twincities\\
        \#breakfast\\
        \emph{Recipe} (recipe, easy, meal)\\
        \#food\\
        i\\
    \end{tabular}
    \caption{        MN }
\end{subtable}
\begin{subtable}{0.25\textwidth}
    \begin{tabular}{l}
        \emph{You, We} (you, we, your, us)\\
        beef\\
        we\\
        \#cwe\\
        fonda\\
        port\\
        us\\
        our\\
        come\\
        wrap\\
    \end{tabular}
    \caption{        MO }
\end{subtable}
\begin{subtable}{0.25\textwidth}
    \begin{tabular}{l}
        \emph{After Work} (time, home, after, work)\\
        \#lunch\\
        TOPIC\_95\\
        \#supper\\
        \#tuesday\\
        \emph{Group Dining} (our, us, join)\\
        join\\
        \#thursday\\
        \#drinkspecials\\
        dispatch\\
    \end{tabular}
    \caption{        MS }
\end{subtable}
\begin{subtable}{0.25\textwidth}
    \begin{tabular}{l}
        TOPIC\_95\\
        chicken\\
        breakfast\\
        when\\
        \#meal\\
        you\\
        out\\
        \emph{I, You} (i, my, you, your)\\
        TOPIC\_129\\
        \#fatburning\\
    \end{tabular}
    \caption{        MT }
\end{subtable}
\begin{subtable}{0.25\textwidth}
    \begin{tabular}{l}
        \#cltfood\\
        \emph{Mixed Drinks} (bottomless mimosas, bloody mary)\\
        bottomless\\
        mimosas\\
        12\\
        10\\
        5churchclt\\
        sunday\\
        sangria\\
        starts\\
    \end{tabular}
    \caption{        NC }
\end{subtable}
\begin{subtable}{0.25\textwidth}
    \begin{tabular}{l}
        \#breakfast\\
        lunch\\
        quick\\
        i\\
        breakfast\\
        til\\
        w\\
        yet\\
        specials\\
        2\\
    \end{tabular}
    \caption{        ND }
\end{subtable}
\begin{subtable}{0.25\textwidth}
    \begin{tabular}{l}
        \emph{Promotional} (free, off, today)\\
        code\\
        promo\\
        off\\
        40\\
        ch40off\\
        your\\
        use\\
        every\\
        2\\
    \end{tabular}
    \caption{        NE }
\end{subtable}
\begin{subtable}{0.25\textwidth}
    \begin{tabular}{l}
        \#recipe\\
        \#follow\\
        TOPIC\_90\\
        4f\\
        \#f\\
        \#followme\\
        pizza\\
        chicken\\
        \#ontheblog\\
        \#tagsforlikes\\
    \end{tabular}
    \caption{        NH }
\end{subtable}
\begin{subtable}{0.25\textwidth}
    \begin{tabular}{l}
        specials\\
        \#restaurant\\
        lunch\\
        \#bestburger\\
        \emph{Group Dining} (our, us, join)\\
        \emph{Japanese} (ramen, japanese, noodles)\\
        \#tapas\\
        \#byob\\
        \#takeout\\
        open\\
    \end{tabular}
    \caption{        NJ }
\end{subtable}
\begin{subtable}{0.25\textwidth}
    \begin{tabular}{l}
        mother\\
        \#trayvonmartin\\
        \#blackhistorymonth\\
        \#kickoff\\
        TOPIC\_133\\
        word\\
        tomorrow\\
        spread\\
        \emph{Mexican} (mexican, tacos, burrito)\\
        my\\
    \end{tabular}
    \caption{        NM }
\end{subtable}
\begin{subtable}{0.25\textwidth}
    \begin{tabular}{l}
        \emph{Restaurant Advertising} (open, today, come, join)\\
        11am\\
        \#happyhour\\
        4pm\\
        3\\
        til\\
        beer\\
        today\\
        \#yummy\\
        my\\
    \end{tabular}
    \caption{        NV }
\end{subtable}
\begin{subtable}{0.25\textwidth}
    \begin{tabular}{l}
        \#brunch\\
        photo\\
        \#dinner\\
        \#food\\
        \#healthy\\
        \#astoria\\
        \emph{Mixed Drinks} (bottomless mimosas, bloody mary)\\
        \emph{Meat} (steak, beef, meat)0\\
        \#sarabeths\\
        w\\
    \end{tabular}
    \caption{        NY }
\end{subtable}
\begin{subtable}{0.25\textwidth}
    \begin{tabular}{l}
        \emph{Airport} (airport, lounge, waiting)\\
        \#plates\\
        \#designer\\
        modern\\
        \#house\\
        \#purple\\
        \#twye\\
        must\\
        \#gray\\
        grace\\
    \end{tabular}
    \caption{        OH }
\end{subtable}
\begin{subtable}{0.25\textwidth}
    \begin{tabular}{l}
        \#cooking\\
        \#lunch\\
        i\\
        \#recipe\\
        chips\\
        come\\
        pickle\\
        \#stellaokc\\
        sub\\
        any\\
    \end{tabular}
    \caption{        OK }
\end{subtable}
\begin{subtable}{0.25\textwidth}
    \begin{tabular}{l}
        \#pdx\\
        \#pdxeats\\
        \#foodlove\\
        \#dairyfree\\
        \#galactosemia\\
        TOPIC\_32\\
        \#instafood\\
        \emph{Restaurant Advertising} (open, today, come, join)\\
        \#foodpics\\
        open\\
    \end{tabular}
    \caption{        OR }
\end{subtable}
\begin{subtable}{0.25\textwidth}
    \begin{tabular}{l}
        great\\
        breakfast\\
        cafe\\
        begun\\
        brunch\\
        \#beatdallas\\
        day\\
        hunt\\
        one\\
        \#eaglesnation\\
    \end{tabular}
    \caption{        PA }
\end{subtable}
\begin{subtable}{0.25\textwidth}
    \begin{tabular}{l}
        specials\\
        new\\
        \#breakfast\\
        topped\\
        \#pancakes\\
        \#yum\\
        TOPIC\_143\\
        \emph{Roasted Meats} (pork, chicken, special)\\
        \#eatclean\\
        \#goodmorning\\
    \end{tabular}
    \caption{        RI }
\end{subtable}
\begin{subtable}{0.25\textwidth}
    \begin{tabular}{l}
        \#chseats\\
        \#chs\\
        TOPIC\_95\\
        \#applebees\\
        \#dmg\\
        \#breastcancerawareness\\
        lunch\\
        \emph{American Diet} (chicken, beans, potatoes)\\
        \emph{First-Person Casual} (my, i, lol)\\
        grits\\
    \end{tabular}
    \caption{        SC }
\end{subtable}
\begin{subtable}{0.25\textwidth}
    \begin{tabular}{l}
        \#snack\\
        tanka\\
        TOPIC\_19\\
        waffle\\
        \#food\\
        \#healthy\\
        locator\\
        find\\
        store\\
        \#supper\\
    \end{tabular}
    \caption{        SD }
\end{subtable}
\begin{subtable}{0.25\textwidth}
    \begin{tabular}{l}
        TOPIC\_32\\
        scones\\
        chocolate\\
        white\\
        \#foodie\\
        specials\\
        morning\\
        \emph{Deli} (cheese, sandwich, soup)\\
        quiche\\
        restaurant\\
    \end{tabular}
    \caption{        TN }
\end{subtable}
\begin{subtable}{0.25\textwidth}
    \begin{tabular}{l}
        my\\
        \emph{Mexican} (mexican, tacos, burrito)\\
        \emph{After Work} (time, home, after, work)\\
        \#tacos\\
        tacos\\
        \#littleblackdress\\
        lol\\
        \#lunch\\
        \#mimosas\\
        TOPIC\_108\\
    \end{tabular}
    \caption{        TX }
\end{subtable}
\begin{subtable}{0.25\textwidth}
    \begin{tabular}{l}
        TOPIC\_117\\
        recipe\\
        \#slc\\
        \emph{Mexican} (mexican, tacos, burrito)\\
        \#rubios\\
        fangram\\
        \#recipe\\
        romantic\\
        \#meal\\
        \#breakfast\\
    \end{tabular}
    \caption{        UT }
\end{subtable}
\begin{subtable}{0.25\textwidth}
    \begin{tabular}{l}
        \#rvadine\\
        \#date\\
        lunch\\
        7\\
        photo\\
        brunch\\
        drink\\
        chicken\\
        \#lunchtime\\
        \#nova\\
    \end{tabular}
    \caption{        VA }
\end{subtable}
\begin{subtable}{0.25\textwidth}
    \begin{tabular}{l}
        \#btv\\
        soup\\
        now\\
        mas\\
        print\\
        fina\\
        today\\
        \#restaurant\\
        \#foods\\
        lunch\\
    \end{tabular}
    \caption{        VT }
\end{subtable}
\begin{subtable}{0.25\textwidth}
    \begin{tabular}{l}
        \#dinner\\
        \#easter\\
        soup\\
        i\\
        \#foodporn\\
        \emph{Meat} (steak, beef, meat)4\\
        \#recipe\\
        recipe\\
        TOPIC\_79\\
        \#foodie\\
    \end{tabular}
    \caption{        WA }
\end{subtable}
\begin{subtable}{0.25\textwidth}
    \begin{tabular}{l}
        \#paleo\\
        \#salad\\
        \#breakfast\\
        \#yum\\
        salad\\
        avocado\\
        \#vegan\\
        chili\\
        some\\
        today\\
    \end{tabular}
    \caption{        WI }
\end{subtable}
\begin{subtable}{0.25\textwidth}
    \begin{tabular}{l}
        \#dinner\\
        card\\
        like\\
        easy\\
        \#yum\\
        \emph{Mexican} (mexican, tacos, burrito)\\
        toast\\
        \emph{Delicious} (foodporn, yummy, yum)\\
        20\\
        \#dinnertime\\
    \end{tabular}
    \caption{        WV }
\end{subtable}
\begin{subtable}{0.25\textwidth}
    \begin{tabular}{l}
        my\\
        \#meal\\
        \#fatburning\\
        \emph{Paleo Diet} (paleo, chicken, healthy)3\\
        \#recipe\\
        \#snack\\
        so\\
        \#fitfam\\
        TOPIC\_32\\
        \#glutenfree\\
    \end{tabular}
    \caption{        WY }
\end{subtable}

\caption{\label{tbl:state_features}Highest-weighted tokens for predicting tweets are from a state.}
\end{table}

